Floorplan Restoration by Structure Hallucinating Transformer Cascades

This paper presents an extreme floorplan reconstruction task, a new benchmark for the task, and a neural architecture as a solution. Given a partial floorplan reconstruction inferred or curated from panorama images, the task is to reconstruct a complete floorplan including invisible architectural structures. The proposed neural network 1) encodes an input partial floorplan into a set of latent vectors by convolutional neural networks and a Transformer; and 2) reconstructs an entire floorplan while hallucinating invisible rooms and doors by cascading Transformer decoders. Qualitative and quantitative evaluations demonstrate effectiveness of our approach over the benchmark of 701 houses, outperforming the state-of-the-art reconstruction techniques. We will share our code, models, and data.

==> module.tex <==
\section{Architecture specifications}

\mysubsubsection{Category Wise CNN} Input for this module is $14\times800\times 800$.
\begin{table}[]
    \centering
    \begin{tabular}{c|c|c}
    
        Layer name &  Specification & Output size  \\ \hline\hline
       Conv1  & $ 7\times7$, 64, stride 2   & $64 \times 400 \times 400$ \\ \hline
       
        \multirow{4}{*}{Conv Block 2} & $3\times 3$, maxpool, stride 2 &    \multirow{4}{*}{$256 \times 200 \times 200$}\\
       &   \multirow{3}{*}{$\left[\begin{array}{l}1 \times 1,64 \\
3 \times 3,64\\  1 \times 1,256\\
 \end{array}\right] \times 3$}   &  \\
          &  & \\
          &  & \\ \hline
          
          
          
          \multirow{3}{*}{Conv Block 3} & 
          \multirow{3}{*}{$\left[\begin{array}{l}1 \times 1,128 \\
3 \times 3,128\\  1 \times 1,512\\
 \end{array}\right] \times 4$}   & \multirow{3}{*}{$512 \times 100 \times 100$} \\
          &  & \\
          &  & \\ \hline
          
          
            \multirow{3}{*}{Conv Block 4} & 
          \multirow{3}{*}{$\left[\begin{array}{l}1 \times 1,256 \\
3 \times 3,256\\  1 \times 1,1024\\
 \end{array}\right] \times 6$}   & \multirow{3}{*}{$1024 \times 50 \times 50$}\\
          &  & \\
          &  & \\ \hline
          
            \multirow{3}{*}{Conv Block 5} & 
          \multirow{3}{*}{$\left[\begin{array}{l}1 \times 1,512 \\
3 \times 3,512\\  1 \times 1,2048\\
 \end{array}\right] \times 3$}   & \multirow{3}{*}{$2048 \times 25 \times 25$}\\
          &  & \\
          &  & \\ \hline
          Conv6  & $ 1\times1$, 256  & $256 \times 25 \times 25$ \\ \hline
          
          
          
    \end{tabular}
    \caption{Category Wise CNN (C-Wise CNN) block}
    \label{tab:my_label}
\end{table}


For the house/apartment with X number of visible rooms, We will have X number of C-wise CNN for rooms were the output will be $X \times 256 \timea 25\times 25$, then we apply max function which result output  of that to be $ \times 256 \timea 25\times 25$. Same with apply to door and room  (both) category, for doors only category there is no need for max.  then we concatenate them resulting output of all to be $3 \times 256\time 25 \time25$, then we reshape them to get input sequence for encoder to be $  1875 \times 256 $ let's call it \emph{src}.  





\mysubsubsection{Encoder}
We have 6 layers of encoder, each layer of that will be as~\ref{tab:table2}


\begin{table}[]
    \centering
    \begin{tabular}{c|c|c|c}
    
        Layer name &  input & Specification & Output size  \\ \hline\hline
        
        Multi head attention & src & embed\_dim=256 , num\_heads=8 &  $1875 \times 256$ (src2)\\
        
        drop out &   src2 & drop out =0.1 & $1875 \times 256$ (src3)\\
        
        LayerNorm & src3+src &   normalized\_shape =256 & $1875 \times 256$ (src4)\\ \hline
        
        
        Linear1, relu & src4 & in\_features=256, out\_features=2048 , &  $1875 \times 2048$ (src5)\\ 
        
         drop out &   src5 & drop out =0.1 & $1875 \times 2048$ (src6)\\
        
        Linear 2 & src6&  in\_features=2048, out\_features=256  &$1875 \times 256 $(src7)
 \\        
         drop out &   src7 & drop out =0.1 & $1875 \times 256$ (src8)\\
        
        LayerNorm & src8+src4 &   normalized\_shape =256 & $1875 \times 256$ (src9)\\ \hline
        
        
    \end{tabular}
    \caption{One layer in encoder, we have 6 layers}
    \label{tab:table2}
\end{table}

Final output of encoder will be $256 \time 1875$ where we only use the one for room-door ones for decoder input which will be $256 \times 625$ lets call this memory(Mem.). 



\mysubsubsection{Decoder}
We have three decoder blocks as~\ref{tab:table3}. Let's assume that we have Y dangling doors. then number of queries for first decoder will be Y, second will be Y+15 and third will be Y+30. Lets show each cascade input queries as "tgt".


\begin{table}[]
    \centering
    \begin{tabular}{c|c|c|c}
    
        Layer name &  input & Specification & Output size  \\ \hline\hline
        
        Multi head attention & tgt & embed\_dim=256 , num\_heads=8 &  $1875 \times 256$ (tgt2)\\
        
        drop out &   tgt2 & drop out =0.1 & $1875 \times 256$ (tgt3)\\
        
        LayerNorm & tgt3+tgt &   normalized\_shape =256 & $1875 \times 256$ (tgt4)\\ \hline
        
        
        Multi head attention & Mem, tgt & embed\_dim=256 , num\_heads=8 &  $1875 \times 256$ (tgt5)\\
        drop out &   tgt6 & drop out =0.1 & $1875 \times 256$ (tgt7)\\
        LayerNorm & tgt7+tgt4 &   normalized\_shape =256 & $1875 \times 256$ (tgt8)\\ \hline
        
        
        
        
        Linear1, relu & tgt8 & in\_features=256, out\_features=2048 , &  $1875 \times 2048$ (tgt9)\\ 
        
         drop out &   tgt9 & drop out =0.1 & $1875 \times 2048$ (tgt10)\\
        
        Linear 2 & tgt10&  in\_features=2048, out\_features=256  &$1875 \times 256 $(tgt11)
 \\        
         drop out &   tgt11 & drop out =0.1 & $1875 \times 256$ (tgt12)\\
        
        LayerNorm & tgt8+tgt11 &   normalized\_shape =256 & $1875 \times 256$ tgt12\\ \hline
        
        
    \end{tabular}
    \caption{One layer in decoder, we have 6 layers}
    \label{tab:table3}
\end{table}


first cascade input is Y dummy queries and encoder output ("Mem"), for second cascade first cascade output will be concatenate with 15 dummy queries and will result in input queries for decoder along with encoder output, for last cascade second cascade output will be concatenate with 15 dummy queries and same as other two it also receives encoder output.



==> qualitative_results.tex <==
\section{More qualitative results}

First in Fig~\ref{fig:sup1}, we show SfM camera pose vs GT camera pose of same samples that we show in figure 5 in main paper, where there we only show GT camera pose version before and after housegan++.




\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/qual_sup1.pdf}
    \caption{SfM and GT camera pose different baseline(related to paper figure 5)}
    \label{fig:sup1}
\end{figure*}

==> sections/diffrent_iou.tex <==




==> sections/subs.tex <==
\newpage

The supplementary document provides backgound on other related datasets and more details on  our dataset~\ref{section:dataset}, the full specifications of our neural architecture in Section~\ref{sec:spec},
more information about loss function~\ref{sec:loss_sup} and computation complexity~\ref{sec:compute} , 
and ~\ref{section:refinment}, results on different IOUs provided in~\ref{fig:IOU} and more experimental results in~\ref{sec:res_sub}.


\input{sections/dataset_sup}
\input{sections/arch}
\input{sections/loss}
\input{sections/computation}
\input{sections/refine}
\input{sections/diffrent_iou}
\input{sections/additional_results}








